Rolling Ball Optimizer: Learning by ironing out loss landscape wrinkles

Training large neural networks (NNs) requires optimizing high-dimensional data-dependent loss functions. The optimization landscape of these functions is often highly complex and textured, even fractal-like, with many spurious local minima, ill-conditioned valleys, degenerate points, and saddle points. Complicating things further is the fact that these landscape characteristics are a function of the data, meaning that noise in the training data can propagate forward and give rise to unrepresentative small-scale geometry. This poses a difficulty for gradient-based optimization methods, which rely on local geometry to compute updates and are, therefore, vulnerable to being derailed by noisy data. In practice,this translates to a strong dependence of the optimization dynamics on the noise in the data, i.e., poor generalization performance. To remediate this problem, we propose a new optimization procedure: Rolling Ball Optimizer (RBO), that breaks this spatial locality by incorporating information from a larger region of the loss landscape in its updates. We achieve this by simulating the motion of a rigid sphere of finite radius rolling on the loss landscape, a straightforward generalization of Gradient Descent (GD) that simplifies into it in the infinitesimal limit. The radius serves as a hyperparameter that determines the scale at which RBO sees the loss landscape, allowing control over the granularity of its interaction therewith. We are motivated by the intuition that the large-scale geometry of the loss landscape is less data-specific than its fine-grained structure, and that it is easier to optimize. We support this intuition by proving that our algorithm has a smoothing effect on the loss function. Evaluation against SGD, SAM, and Entropy-SGD, on MNIST and CIFAR-10/100 demonstrates promising results in terms of convergence speed, training accuracy, and generalization performance.

==> assets/figures/tikz/sharpvflat.tex <==

\definecolor{c2000f6}{RGB}{32,0,246}
\definecolor{c00ff6e}{RGB}{0,255,110}
\definecolor{ccc0000}{RGB}{204,0,0}
\definecolor{c0000b8}{RGB}{0,0,184}


\def \globalscale {1.000000}
\begin{tikzpicture}[y=1cm, x=1cm, yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}, inner sep=0pt, outer sep=0pt]
	\path[draw=black,line cap=butt,line join=miter,line width=0.03cm,<-] (8.599, 0.9146) -- (0.7938, 0.9146);



	\path[draw=black,line cap=butt,line join=miter,line width=0.0265cm,<-] (0.7938, 6.341) -- (0.7938, 0.9146);



	\path[draw=black,line cap=butt,line join=miter,line width=0.0265cm] (1.1906, 5.1479).. controls (1.3469, 3.7897) and (1.5875, 1.576) .. (3.0427, 1.576).. controls (4.4979, 1.576) and (5.6605, 3.7841) .. (5.9531, 5.1479).. controls (6.2177, 3.6927) and (6.4823, 1.576) .. (7.1438, 1.576).. controls (7.8208, 1.5595) and (7.8052, 3.6927) .. (7.9375, 5.1479);



	\path[draw=c2000f6,line cap=butt,line join=miter,line width=0.0265cm,miter limit=4.0,dash pattern=on 0.106cm off 0.053cm] (1.9833, 5.1479).. controls (2.1395, 3.7897) and (2.3801, 1.576) .. (3.8353, 1.576).. controls (5.2906, 1.576) and (6.4531, 3.7841) .. (6.7458, 5.1479).. controls (7.0103, 3.6927) and (7.2749, 1.576) .. (7.9364, 1.576).. controls (8.6134, 1.5595) and (8.5978, 3.6927) .. (8.7301, 5.1479);



	\node[text=black,line width=0.0091cm,anchor=south west] (text2683) at (3.4185, 0.4064){Parameter value};



	\node[text=black,line width=0.011cm,rotate=90.0,anchor=south west] (text5009) at (0.5503, 2.3904){Loss function};



	\path[draw=c00ff6e,line cap=butt,line join=miter,line width=0.0265cm,miter limit=4.0,dash pattern=on 0.0265cm off 0.0265cm] (3.0427, 1.8406) -- (3.0427, 0.9146);



	\path[draw=black,line cap=butt,line join=miter,line width=0.0265cm,miter limit=4.0,dash pattern=on 0.0265cm off 0.0265cm] (3.0427, 1.576) -- (0.7938, 1.576);



	\path[draw=c00ff6e,line cap=butt,line join=miter,line width=0.026cm,miter limit=4.0,dash pattern=on 0.026cm off 0.026cm] (3.0427, 1.8406) -- (0.7938, 1.8406);



	\path[draw=ccc0000,line cap=butt,line join=miter,line width=0.0265cm,miter limit=4.0,dash pattern=on 0.0265cm off 0.0265cm] (7.1438, 0.9146) -- (7.1438, 3.0313);



	\path[draw=black,fill=cyan,line cap=butt,line join=miter,line width=0.0265cm,miter limit=4.0,dash pattern=on 0.0265cm off 0.0265cm] (7.1438, 1.576) -- (0.7938, 1.576);



	\path[draw=ccc0000,line cap=butt,line join=miter,line width=0.0265cm,miter limit=4.0,dash pattern=on 0.0265cm off 0.0265cm] (7.1438, 3.0313) -- (0.7938, 3.0313);



	\path[even odd rule,line width=0.0149cm,miter limit=4.0,cm={ 1.4443,-0.0,-0.0,1.4443,(-4.3339, 2.3747)}] (3.8365, 2.6344) -- (3.8365, 2.0391) -- (5.0271, 2.0391) -- (5.0271, 2.6344) -- cycle;



	\path[draw=black,line cap=butt,line join=miter,line width=0.0287cm] (1.3505, 5.8928) -- (1.7804, 5.8928);



	\path[draw=c0000b8,line cap=butt,line join=miter,line width=0.0287cm,miter limit=4.0,dash pattern=on 0.086cm off 0.0287cm] (1.3505, 5.6062) -- (1.7804, 5.6062);



	\node[text=black,line width=0.0054cm,anchor=south west] (text14979) at (1.9645, 5.8436){Training};



	\node[text=black,line width=0.0054cm,anchor=south west] (text14979-3) at (1.9623, 5.5357){Testing};




\end{tikzpicture}


==> description.tex <==
\section{Model description and theoretical analysis}\label{sec:description}

\subsection{Theoretical analysis}\label{sub:description:analysis}

In \Cref{sec:intuition}, we motivated the rolling ball optimizer
by the empirical observation that the trajectories of objects with non-zero dimensions
are invariant to the microscopic topography of the surface they are rolling on
in a way that infinitesimal point particles are not.
Having defined the rolling ball optimizer in \Cref{sub:description:description},
we observe a property which makes this intuition rigorous:
the sequence of centers \((c_{t})_{t \ge 0}\) maintains a constant distance from \(\Gamma\).
i.e.,
\begin{equation}\label{eq:offset-manifold}
	\forall t \ge 0, \quad d(c_{t}, \Gamma) \coloneqq
	\min_{p\in\Gamma}{\norm{c_{t} - p}} = \norm{c_{t} - p_{t}} = r.
\end{equation}
The centers are confined to the \emph{\(r-\)offset manifold} of \(\Gamma\),
which can be seen as a smoothed version of \(\Gamma\), getting smoother as \(r\) increases.
This corresponds to bigger balls being robust to larger-scale details of the loss landscape.


\paragraph{Problems so far}

\begin{enumerate}
	\item The footpoint projection problem:
	      \begin{enumerate}
		      \item It involves \(f\), and \(\grad{f}\) at each iteration.
		      \item The projection is not guaranteed to be unique.
		      \item It is not clear what the projection is when the ball is not tangent to \(\Gamma\).
	      \end{enumerate}
	\item Smoothness of the manifold of centers:
	      \begin{enumerate}
		      \item The offset manifold seems not to be the right object to study.
		      \item The true locus of centers seems difficult to characterize.
	      \end{enumerate}
	\item What to do if the ball finds itself in a tight valley (it must go through the walls)?
\end{enumerate}

\paragraph{Potential solutions}
\begin{enumerate}
	\item The footpoint projection problem:
	      \begin{enumerate}
		      \item We can use single batch evaluations of \(f\) and \(\grad{f}\) per iteration.
		      \item We can initialize the projection with some function of the previous iterate,
		            and use a small \(\eta\) to get the projection in the direction we came from.
		            The other footpoints can be ignored. This can even be seen as a form of momentum.
		            However, it becomes necessary to test whether the center is above or below \(\Gamma\).
	      \end{enumerate}
	\item Smoothness of the manifold of centers:
	      \begin{enumerate}
		      \item For simple cases (e.g., a parabola),
		            we can try to characterize the locus of centers explicitly.
		      \item Computer graphics and physics engines can be used
		            to simulate the rolling ball optimizer and study the locus of centers.
	      \end{enumerate}
	\item Depending on the height of the valley, we can either ignore it, or fail.
	      This appears to be a true limitation of the optimizer. Another one is plateau regions.
\end{enumerate}

==> limitations.tex <==
\section{Limitations and future work}\label{sec:limitations}

Despite the promising empirical results, as well as the theoretical insights presented in this work,
several challenges remain to be addressed.
In this section, we present a number of limitations,
and suggest potential directions for addressing them.


% \subsection{Computational cost}\label{sub:complexity}

% To compare the computational cost of different optimizers,
% we will measure runtime in terms of the number of passes (forward and backward)
% through the loss function, and memory footprint in terms of the number of models to store.
% Standard variants of \gls{abb:sgd}, including adaptive methods and momentum-based methods,
% only require two passes through the loss function per epoch.
% Similarly, they only require a constant amount of memory to store the model and the optimizer state.

% Both our optimizers on the other hand, have a higher time complexity.
% The rolling ball optimizer requires \(\bigO{\left( n_{\text{iter}} \right)}\)
% passes per epoch, to perform the projections, while the position-based dynamics optimizer
% needs to solve \(\frac{n_{\text{vert}}(n_{\text{vert}}-1)}{2}\) constraints,
% requiring \(n_{\text{proj}}\) iterations each.
% % ! this is an important realization
% This does not contribute to our measure of number of passes
% because the constraints do not involve the loss function.

% In terms of memory footprint, the rolling ball is identical to \gls{abb:sgd},
% while the position-based dynamics optimizer requires storing all the vertices.
% To make things more complicated, the number of vertices required to
% uniquely describe the sphere grows linearly with the dimension of the space.


% % Sliding ball optimization requires nested optimization loops, making it computationally expensive.
% % This is due to the complex nature of \(\Gamma\), which doesn't have an efficient
% % projection operator or distance estimator.
% % The most obvious solution to this problem is to approximate \(\Gamma\) with a simpler manifold.
% % In particular, for small values of \(\eta\), the next footpoint is close to the current one,
% % meaning that projecting on the tangent hyperplane at the current footpoint is a good approximation.
% % This has the major benefit of requiring no iterative optimization, nor additional passes through \(f\).
% % Another approach is, to look for a footpoint on the line segment
% % connecting the current footpoint to the candidate center.
% % This can be done by solving a one-dimensional root-finding problem,
% % requiring only a logarithmic number of evaluations of \(f\) (and no gradient evaluations).


% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{lcc}
% 			\toprule
% 			\textbf{Algorithm} & \textbf{Time Complexity}                                         & \textbf{Space Complexity}               \\
% 			\midrule
% 			\gls{abb:sgd}      & \(\bigO{\left(n_{\text{epochs}}\right)}\)                        & \(\bigO{(1)}\)                          \\
% 			RBO                & \(\bigO{\left(n_{\text{epochs}} \times n_{\text{iter}}\right)}\) & \(\bigO{(1)}\)                          \\
% 			PBDO               & \(\bigO{\left(n_{\text{epochs}} \right)}\)                       & \(\bigO{\left(n_{\text{vert}}\right)}\) \\
% 			\bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{Comparison of runtime and memory footprint scaling for different optimization algorithms.}%
% 	\label{tab:complexity}
% \end{table}


% \subsection{Variants and extensions}\label{sub:variants}

% Both of the optimizers discussed in this work can be modified in several ways.
% We list a few possible extensions here.

% \begin{enumerate}
% 	\item \textbf{Rolling ball optimizer.}
% 	      For small values of \(\eta\), the next footpoint is close to the current one.
% 	      Projection on the tangent hyperplane at the current footpoint is a good approximation.
% 	      This has the notable advantage of requiring no additional work,
% 	      bringing the time complexity of the optimizer down to that of \gls{abb:sgd}.
% 	\item \textbf{Position-based dynamics optimizer.}
% 	      \begin{enumerate}
% 		      \item \textbf{Multiple elasticities.}
% 		            So far we operated on the assumption that all constraints have the same elasticity.
% 		            This is not necessary, as any symmetric matrix can be used as the elasticity matrix.
% 		      \item \textbf{Loss-aware distance.}
% 		            The vertices live in parameter space.
% 		            Their motion is analogous to the motion of the ball's shadow.
% 		            This is not a problem if we have enough vertices to uniformly describe the sphere,
% 		            but if not, rigid motion in ambient space may not result in a rigid shadow.
% 		            This can be addressed by using a loss-aware distance metric.
% 		            The Euclidean distance in ambient space is a possible choice,
% 		            and so is the geodesic distance on \(\Gamma\).
% 	      \end{enumerate}
% 	\item \textbf{Both.}
% 	      Both algorithms may benefit from using schedules for the hyperparameters.
% 	      This includes the step sizes, but also the number of projection iterations.
% \end{enumerate}


==> method.tex <==
\section{Method}\label{sec:method}

Consider a typical \gls{abb:dl} training setup,
where we seek to minimize a positive, differentiable loss function \(f:\reals^{d} \to \reals\),
using \gls{abb:gd}
\begin{equation}\label{eq:gd}
	\theta_{t+1} = \theta_{t} - \eta \grad{f}{(\theta_{t})},
\end{equation}
where \(\eta > 0\) is the learning rate.
The graph of \(f\), i.e., the set \(\Gamma = \left\{ (\theta, f(\theta)) \middle| \theta \in \reals^{d} \right\}\)
is a \((d+1)\)-dimensional submanifold of \(\reals^{d} \times \reals \iso \reals^{d+1}\),
which we will refer to as the \emph{loss manifold}, \emph{loss surface}, or \emph{loss landscape}.
The iterates produced by \gls{abb:gd} are analogous%
\footnote{%
	A physicist might -- rightfully -- object to this analogy,
	on the grounds that the training dynamics take the form
	\(\dot{\theta} \propto F(\theta)\) rather than \(\ddot{\theta} \propto F(\theta, \dot{\theta})\).
	However, it turns out that the discrete nature of \gls{abb:gd} gives rise to
	a form of \emph{implicit acceleration}~\citep{tanakaNoethersLearningDynamics2021}.
}
to the successive positions of a point particle
%! The fact that it's constrained to \(\Gamma\) can be seen as a constraint (holonomic)
moving on \(\Gamma\), subject to a force field in the direction of \(-\grad{f}{(\theta)}\).
Equilibria of this system correspond to the critical points of \(f\)
(assuming no momentum, nor gradient noise),
and stable equilibria correspond to local minima.
The particle gets stuck at the first minimum it encounters.

\subsection{Motivating intuition}\label{sub:method:intuition}

\Gls{abb:gd}'s behavior as described above is undesirable,
as the loss landscape is almost always non-convex,
exhibiting many local minima of differing quality, as well as maxima and saddle points.
Furthermore, the loss landscape is often very rough, with minima packed closely together,
making it unlikely for the particle to move far from its initial position,
%todo: see if ypu can find proof that every initial position is close to a minimum
a phenomenon known as \emph{lazy training}~\citep{chizatLazyTrainingDifferentiable2019}.
This latter issue is particularly problematic,
as it means that the learned parameters
are extremely dependent on the fine-grained topography of the loss landscape,
which is in turn very dependent on the training data (and the noise therein),
making overfitting more likely.
On top of that, the complicated geometry of the loss landscape
makes it extremely challenging to predict the trajectory of the iterates, even qualitatively.

The root of the problem is in the point-like, zero-dimensional nature of the particle,
which allows it to be trapped in an arbitrarily small and sharp valley.
An object with non-zero dimensions, such as a marble or a ball, on the other hand,
can't be trapped in a basin smaller than its diameter.
%todo: I belive there is a phase transition 
% with criticality at the point wher ball is smaller than % the smallest basin. 
% At this point, it will behave like a point particle.
It ignores the microscopic valleys and hills, and heads straight for the bottom of the basin it's in.
In this way, it is far more robust to insignificant changes in the training data,
and thus more likely to generalize well.
Therefore, it stands to reason that an optimizer which mimics the behavior of such an object
would be more resilient to loss landscape pathology than one that behaves like a point particle.

\subsection{Rolling ball optimizer}\label{sub:method:rbo}

Instead of the successive positions of a point particle,
let the iterates describe the location of a finite-sized object moving in \(\reals^{d}\).
For the sake of simplicity, we will consider the object is completely rigid
(we relax this restriction in~\Cref{sub:method:pbo}),
so that its position is uniquely determined by its orientation and its center.
To further simplify the problem, we suppose that the object is spherical,
which allows us to ignore orientation.

In order to derive a physically plausible update rule,
first, consider the \(t^\text{th}\) iterate \(\theta_{t}\in\reals^{d}\).
The center \(c_{t}\) of the ball of radius \(r>0\),
tangent to \(\Gamma\) at \(p_{t}=(\theta_{t}, f(\theta_{t}))\),
is given by
\begin{equation}\label{eq:center}
	c_{t} = p_{t} + r n_{t},
\end{equation}
where \(n_{t}\) is the unit normal to \(\Gamma\) at \(p_{t}\),
in turn given by
\begin{equation}\label{eq:normal}
	n_{t} = \frac{1}{\sqrt{1+\norm{\grad{f}{(\theta_{t})}}^{2}}}
	\begin{bmatrix}
		-\grad{f}{(\theta_{t})} \\ 1
	\end{bmatrix}.
\end{equation}
To simulate one time step of the ball's motion (to get \(c_{t+1}\)),
we take a step of size \(\eta\) along\(\tau_{t}\):
\begin{equation}\label{eq:candidate}
	\tilde{c}_{t+1} = c_{t} - \eta \tau_{t},
\end{equation}
where \(\tau_{t}\) is the tangent vector to \(\Gamma\) at \(p_{t}\), given by
\begin{equation}\label{eq:tangent}
	\tau_{t} = \begin{bmatrix}
		\grad{f}{(\theta_{t})} \\ \norm{\grad{f}{(\theta_{t})}}^{2}
	\end{bmatrix},
\end{equation}
giving us a candidate \(\tilde{c}_{t+1}\) for the next center.
The reason why \Crefformat{eq:candidate} yields a candidate rather than the actual center
is that sphere of radius \(r\) centered at \(\tilde{c}_{t+1}\) may not be tangent to \(\Gamma\).
We therefore project \(\tilde{c}_{t+1}\) onto \(\Gamma\) to find is \emph{footpoint} \(p_{t+1}\):
\begin{equation}\label{eq:footproject}
	\begin{split}
		p_{t+1} & = \argmin_{p\in\Gamma}{\norm{p - \tilde{c}_{t+1}}}      \\
		        & = \argmin_{p\in\Gamma}{\norm{p - \tilde{c}_{t+1}}^{2}},
	\end{split}
\end{equation}
the \(\theta\) component of which is the \(t+1\) iterate \(\theta_{t+1}\).
This process is illustrated in \Cref{fig:rolling-ball}.
\begin{figure}[hbt]
	\begin{center}
		\begin{asy}
			import graph;
			size(250, 0);

			real radius = 0.2;
			real eta = 0.3;

			xaxis("\(\theta\)", 0, 2);
			yaxis("\(f(\theta)\)", 0, 1);

			pair f(real x) { return (x, (x-1)^2); }
			pair ftan(real x) { return (1, 2*(x-1)); }
			pair fperp(real x) { return (2*(x-1), -1)/sqrt(1+4*(x-1)^2); }


			draw(graph(f, 0, 2));

			// initial point
			real theta0 = 1.8;
			pair p0 = f(theta0);
			dot(p0);
			label("\(p_{t}\)", p0, E);
			draw(p0 -- (theta0, 0), dashed);
			label("\(\theta_{t}\)", (theta0, 0), S);

			pair n0 = fperp(theta0);
			pair t0 = ftan(theta0);
			pair c0 = p0 - radius*n0;

			draw(circle(c0, radius), blue);
			draw(p0--c0, red, arrow=ArcArrow(size=2));
			pair candidate = c0 - eta*t0;
			draw(c0--candidate, green, arrow=ArcArrow(size=2));
			draw(circle(candidate, radius), dashed+orange);

			// footpoint
			// real theta1 = 1.34627684058781;
			real theta1 = 1.41;
			pair p1 = f(theta1);
			dot(p1);
			// label("\(p_{t+1}\)", p1, N);
			draw(p1 -- (theta1, 0), dashed);
			label("\(\theta_{t+1}\)", (theta1, 0), S);

			pair n1 = fperp(theta1);

			pair c1 = p1 - radius*n1;
			draw(circle(c1, radius), blue);
			draw(p1--c1, red, arrow=ArcArrow(size=2));


		\end{asy}
	\end{center}
	\caption{One update step of the rolling ball optimizer.}\label{fig:rolling-ball}
\end{figure}

As a matter of fact, we do not need to compute \(p_{t+1}\) entirely, only its \(\theta\) component.
To do so, we rewrite \Cref{eq:footproject} in terms of \(\theta\):
first, let \(\tilde{c}_{t+1} = (\uglytilde{\theta}, \tilde{y})\)
and \(p_{t+1} = (\theta_{t+1}, f(\theta_{t+1}))\).
Then, \Cref{eq:footproject} becomes
\begin{equation}\label{eq:footprojectparam}
	\theta_{t+1} = \argmin_{\theta\in\reals^{d}}%
	{\left[ g(\theta) \coloneqq
			\norm*{\theta - \uglytilde{\theta}}^{2} + \left( f(\theta) - \tilde{y} \right)^{2} \right]}.
\end{equation}
In turn, \Cref{eq:footprojectparam} can be solved using \gls{abb:gd} with step size \(\epsilon\),
and the gradient of \(g\) is given by
\begin{equation}\label{eq:footgrad}
	\grad{g}{(\theta)} = \left( \theta - \uglytilde{\theta} \right) + \left( f(\theta) - \tilde{y} \right) \grad{f}{(\theta)}.
\end{equation}
This entire process (finding a center, taking a step, and projecting)
can be iterated to construct successive centers and footpoints, as shown in \Cref{algo:rolling-ball},
where the \texttt{project} function is defined by \Cref{algo:footpoint-projection}.
\begin{algorithm}[hbt]
	\caption{Rolling ball optimizer}\label{algo:rolling-ball}
	\SetKwFunction{proj}{project}
	\KwIn{
		Loss function \(f:\mathbb{R}^{d} \to \mathbb{R}\) \newline
		Learning rate \(\eta > 0\) \newline
		Ball radius \(r > 0\) \newline
		Initial solution \(\theta_{0} \in \mathbb{R}^{d}\) \newline
		Number of epochs \(n_{\text{epochs}} \ge 1\)
	}
	\Begin{
		\(\theta \leftarrow \theta_{0}\)\;
		\For{\(t = 0\) \KwTo \(n_{\text{epochs}}\)}{
			\(\delta_{t} \leftarrow \grad{f}{(\theta)}\)\;
			\(\tau_{t} \leftarrow \begin{bmatrix} \delta_{t} \\ \norm{\delta_{t}}^{2} \end{bmatrix}\)\;
			\(n_{t} \leftarrow \frac{1}{\sqrt{1 + \norm{\delta_{t}}^{2}}}
			\begin{bmatrix} -\delta_{t} \\ 1 \end{bmatrix}\)\;
			\(c_{t} \leftarrow \theta + r n_{t}\)\;
			\(\tilde{c}_{t+1} \leftarrow c_{t} - \eta \tau_{t}\)\;
			\(\theta_{t+1} \leftarrow\) \proj{\(\tilde{c}_{t}, f\)}\;
		}
	}
	\KwOut{Optimal solution \(\theta^{\ast}\)}
\end{algorithm}
\begin{algorithm}[hbt]
	\caption{Footpoint projection}\label{algo:footpoint-projection}
	\KwIn{
		Function \(f:\mathbb{R}^{d} \to \mathbb{R}\) \newline
		Point \(p = (\theta_{p}, y_{p}) \in \mathbb{R}^{d+1}\) \newline
		Initial solution \(\theta_{0} \in \mathbb{R}^{d}\) \newline
		Step size \(\epsilon > 0\) \newline
		Number of iterations \(n_{\text{iter}} \ge 1\)
	}
	\SetKwProg{Fn}{Function}{:}{end}
	\Fn(\atcp{Projects \(p\) on the graph of \(f\)}){project(\(f, p\))}{
	\(\theta_{q}^{(0)} \gets \theta_{0}\)\;
	\For{\(k = 0\) \KwTo \(n_{\text{iter}}\)}{
		\(y_{q}^{(k)} \gets f(\theta_{q})\)\;
		\(
		\theta_{q}^{(k+1)} \gets \theta_{q}^{(k)} - \epsilon \grad{g}{\left( \theta_{q}^{(k)} \right)}
		\)\tcp*{See \Cref{eq:footgrad}}

	}
	\KwRet{\(\theta_{q}^{(n_{\text{iter}})}\)}
	}
	\KwOut{%
		\(\theta_{q}\), the \(\theta\) coordinate
		of the footpoint of \(p\) on the graph of \(f\).
	}
\end{algorithm}

\begin{figure}[hbt]
	\begin{center}
		\includegraphics[width=0.5\linewidth]{pdf/ball_trajectory}
	\end{center}
	\caption{Trajectory of the rolling ball optimizer for
		\(f(\theta) = \theta^{2}, \theta_{0} = 1, \eta = \epsilon = 0.1,
		r = 0.2, n_{\text{epochs}} = n_{\text{iter}} = 10\).
	}\label{fig:ball_trajectory}
\end{figure}


% \subsection{Position-based optimizer}\label{sub:method:pbo}

% The implementation discussed in~\Cref{sub:method:rbo} is conceptually simple
% by virtue of the idealizations we made (rigidity and sphericity).
% In this section, we consider a more general implementation,
% based on the discrete model of a rigid body, which can handle elastic objects.
% While this method can handle non-spherical objects too, the computations are completely intractable.
% In fact, even for spherical objects,
% we can only handle low-dimensional projections of the ball rather than the ball itself.
% Ultimately, this goes to show that the previous implementation is the most practical one.


% Let \(\left\{ \theta_{t}^{(i)} \in \reals^{d} \middle| i = 1, \ldots, n \right\}\)
% be the \(\theta\) coordinates of \(n_{\text{vert}}\) \emph{vertices}
% defining an object moving on \(\Gamma\).
% The motion of the object is determined by the motion of these vertices.
% The object is rigid if the distance matrix
% \[D_{t} = \left[ \norm*{\theta_{t}^{(i)} - \theta_{t}^{(j)}} \right]_{1\le i,j\le n_{\text{vert}}}\]
% is constant, i.e., \(D_{t+1} = D_{t}\).
% This gives a straightforward way to update the positions:
% \begin{enumerate}
% 	\item Update each vertex \(\theta_{t}^{(i)}\) independently using \gls{abb:gd},
% 	      to get \emph{proposed} positions \(\uglytilde{\theta}_{t+1}^{(i)}\).
% 	\item Enforce the constraint \(D_{t+1} = D_{t}\) using a constraint solver to get the updated
% 	      positions \(\theta_{t+1}^{(i)}\).
% \end{enumerate}
% For the second step, we can use \gls{abb:pbd}, introduced by~\cite{mullerPositionBasedDynamics2007}.
% In essence, \gls{abb:pbd} enforces distance constraints by allowing the vertices
% to attract or repel each other, as if they were connected by springs.
% More precisely, given two proposed positions \(\uglytilde{\theta}_{1}\) and \(\uglytilde{\theta}_{2}\),
% and a desired distance \(d\), constraint projection is done by repeatedly applying
% \begin{equation}\label{eq:pbd}
% 	\begin{split}
% 		\uglytilde{\theta}_{1}^{[s+1]} = \uglytilde{\theta}_{1}^{[s]} + k \Delta^{[s]} \\
% 		\uglytilde{\theta}_{2}^{[s+1]} = \uglytilde{\theta}_{2}^{[s]} - k \Delta^{[s]}
% 	\end{split}, \quad 0 \le s \le n_{\text{proj}},
% \end{equation}
% where \(0\lt k \lt 1\) is a hyperparameter representing the stiffness of the spring,
% \(n_{\text{proj}}\) is the number of projection steps,
% and
% \begin{equation}\label{eq:hookcorrection}
% 	\Delta^{[s]} = \frac{1}{2}
% 	\left( \norm{\uglytilde{\theta}_{1}^{[s]} - \uglytilde{\theta}_{2}^{[s]}} - d \right)
% 	\frac{\uglytilde{\theta}_{1}^{[s]} - \uglytilde{\theta}_{2}^{[s]}}%
% 	{\norm{\uglytilde{\theta}_{1}^{[s]} - \uglytilde{\theta}_{2}^{[s]}}}
% \end{equation}
% is a distance dependent correction (restoring force).
% By varying \(k\), we can control the elasticity of the object,
% \(k=1\) corresponding to a completely rigid object (analogous to a solid),
% and \(k=0\) to an unbound set of vertices (analogous to a fluid).

% Similar to \cite{zhangDeepLearningElastic2015,nelderSimplexMethodFunction1965}.


==> preamble/bibliography.tex <==
\usepackage[sort&compress,numbers]{natbib}                                % Bibliography
\renewcommand{\bibsection}{\section*{References}} % Bibliography title
% \biboptions{sort&compress}                        % Sort and compress citations [1,2,3] -> [1-3]
\bibliographystyle{elsarticle-num-names}          % Bibliography style


==> preamble/code.tex <==
\usepackage{minted}
% \usemintedstyle{native}
\setminted{%
  frame=lines,%
  framesep=2mm,%
  baselinestretch=1.2,%
  % bgcolor=DarkGray,%
  fontsize=\footnotesize,%
  linenos,%
  breaklines,%
}

\renewcommand{\listingscaption}{Code snippet}
\renewcommand{\listoflistingscaption}{List of code snippets}

==> preamble/hyperref.tex <==
\usepackage{hyperref}
\usepackage{cleveref}

\definecolor{CiteBlue}{HTML}{50A8C6}
\definecolor{Link}{named}{DarkBlue}

\makeatletter
\hypersetup{%
	colorlinks=true,
	linkcolor=Link,
	citecolor=CiteBlue,
	urlcolor=blue,
	% pagecolor=red,
	pdfkeywords={Machine Learning, Data Quality, Loss Landscape Analysis},
	pdfauthor={Mohammed D. Belgoumri, Mohamed R. Bouadjenek, Hakim Hacid, Sunil Aryal},
	pdftitle={Loss landscape analysis: State of the art and future directions}
}

% Cleveref formats
\crefformat{principle}{principle.~#2#1#3}
\crefformat{conjecture}{conjecture.~#2#1#3}
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}


==> preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}

Throughout this paper, we consider the typical \gls{abb:dl} training setup
of minimizing a positive (\(k\) times continuously) differentiable loss function \(f: \reals^d \to \reals\),
\(d\) being the parameter space dimension.
The graph of \(f\), i.e., the set
\(\Gamma = \left\{ (\theta, f(\theta)) \middle| \theta \in \reals^{d} \right\}\),
is a (\(\classC^k\)) smooth \(d\)-dimensional submanifold of \(\reals^{d} \times \reals \iso \reals^{d+1}\).
We refer to \(\Gamma\) as the \emph{loss manifold}, \emph{loss surface}, or \emph{loss landscape},
to \(\reals^{d}\) as the \emph{parameter space}, and to \(\reals^{d+1}\) as the \emph{ambient space}.
\(\Gamma\) is naturally parametrized by the mapping \(\theta \mapsto (\theta, f(\theta))\),
which defines a \(\classC^k\)-diffeomorphism between \(\reals^{d}\) and \(\Gamma\).
\(\Gamma\) is therefore orientable, and thus admits a continuous unit normal vector field \(\nu\)
given by
\begin{equation}
	\label{eq:normal}
	p = (\theta, f(\theta)) \mapsto
	\nu(p) = \frac{1}{\sqrt{1 + \norm*{\grad{f}{(\theta)}}^{2}}}
	\begin{bmatrix} -\grad{f}{(\theta)} \\ 1 \end{bmatrix},
\end{equation}
On account of its smoothness, \(\Gamma\) also admits a continuous tangent vector field \(\tau\) given by
\begin{equation}
	\label{eq:tangent}
	p = (\theta, f(\theta)) \mapsto
	\tau(p) = \begin{bmatrix} \grad{f}{(\theta)} \\ \norm*{\grad{f}{(\theta)}}^{2} \end{bmatrix}.
\end{equation}


\subsection{Offset manifolds and tubular neighborhoods}\label{sub:offset-manifolds}

For any point \(p \in \reals^{d+1}\), the distance of \(p\) to \(\Gamma\) is defined as
\begin{equation}
	\label{eq:distance}
	d_{\Gamma}(p) = \inf\limits_{q \in \Gamma} \norm*{p - q}
\end{equation}
The sublevel sets of the function \(d_{\Gamma}\)
are referred to as \emph{tubular neighborhoods} of \(\Gamma\).
More precisely, for \(\rho > 0\), the \(\rho\)-tubular neighborhood of \(\Gamma\) is the set
\begin{equation}
	\label{eq:tubular-neighborhood}
	d_{\Gamma}^{-1}([0, \rho[) \coloneqq
	\left\{ p \in \reals^{d+1} \middle| d_{\Gamma}(p) < \rho \right\},
\end{equation}
or equivalently, the set
\begin{equation}
	\label{eq:tubular-neighborhood-2}
	\bigcup_{p \in \Gamma} \ball{(p, \rho)},
\end{equation}
where \(\ball{(p, \rho)}\) is the open ball of radius \(\rho\) centered at \(p\)%
~\cite{chazalInferenceCurvatureUsing2017}.
The boundary of the tubular neighborhood, or equivalently the level set \(d_{\Gamma}^{-1}(\{\rho\})\),
is referred to as the \(\rho\)-\emph{offset manifold} of \(\Gamma\),
and is denoted by% 
\footnote{%
	In reality, the boundary has two connected components,
	one of which is above the loss landscape.
	We will denote it by \(\Gamma_\rho\),
	and refer to it, by abuse of language, as the \(\rho\)-\emph{offset} of \(\Gamma\).
}
\(\Gamma_\rho\).
It is easy to see that \(\Gamma_\rho\) is also a \(d\)-dimensional submanifold of \(\reals^{d+1}\),
and that it is \(\classC^k\)-diffeomorphic to \(\Gamma\) for small enough \(\rho\)%
~\cite{chazalInferenceCurvatureUsing2017}.

\subsection{Projecting onto a manifold}\label{sub:manifold-projection}

Since \(\Gamma\) is closed, for any point \(p \in \reals^{d+1}\),
there exists a point \(q \in \Gamma\) such that \(\norm*{p - q} = d_{\Gamma}(p)\).
The set of all such points is called the \emph{projection} of \(p\) onto \(\Gamma\),
denoted by \(\project_{\Gamma}(p)\)%
~\citep{%
	chazalInferenceCurvatureUsing2017,%
	leobacherExistenceUniquenessRegularity2021%
}.
The set of points \(p\in\reals^{d+1}\) such that \(\project_{\Gamma}(p)\)
has at least two elements is called the \emph{medial axis} of \(\Gamma\)%
~\cite{%
	chazalInferenceCurvatureUsing2017,%
	leobacherExistenceUniquenessRegularity2021%
}.
Using the projection operator on the updates or iterates of gradient descent,
we obtain a new algorithm whose iterates are confined to a certain manifold (typically, an offset of \(\Gamma\)).
This algorithm is referred to as \gls{abb:pgd}~\citep{hauswirthProjectedGradientDescent2016}.

% \subsection{Dynamics of point particles and rigid bodies}\label{sub:preliminaries:dynamics}

% \Gls{abb:gd} defines a dynamical system on the parameter space \(\reals^{d}\)
% given by the transition function
% \begin{equation}
% 	\label{eq:preliminaries:gd-parameter-space}
% 	\theta_{t+1} = \theta_{t} - \eta \grad{f}{(\theta_{t})},
% \end{equation}
% with the corresponding ambient space dynamics
% \begin{equation}
% 	\label{eq:preliminaries:gd-ambient-space}
% 	p_{t+1} = p_{t} - \eta \tau(p_{t}).
% \end{equation}
% The continuous-time version of \Cref{eq:preliminaries:gd-ambient-space,eq:preliminaries:gd-parameter-space}




==> related.tex <==
\section{Related work}\label{sec:related}

Despite there being, to the best of our knowledge, no explicit distinction in the literature
between point-like or spatially local optimizers on one hand,
and non-local optimizers on the other,
\gls{abb:rbo} is not the first non-local optimizer.
A particularly prominent (and one of the earliest) examples
is Entrpy-\gls{abb:sgd}~\citep{chaudhariEntropySGDBiasingGradient2019},
which is also equivalent to applying \gls{abb:sgd} to a smoothed version of the loss landscape.
Averaged Gradient Descent (AGD)~\citep{biroliHowIronOut2020} is another non-local optimizer,
which operates by averaging the gradient over multiple parameter values.
An interestingly ambiguous case is \gls{abb:sam}~\citep{foretSharpnessawareMinimizationEfficiently2020},
since, as it is defined, it is a non-local optimizer,
but the way it is computed is approximated by a point-like optimizer.
Trust region methods (and by extension, the proximal point method)
are also, by definition, non-local optimizers.
Beyond optimization, this work shares a common physical inspiration
to the rolling ball algorithm from image processing~\citep{sternbergBiomedicalImageProcessing1983}.
